A Framework of High-Stakes Algorithmic Decision-Making for the Public Sector Developed through a Case Study of Child-Welfare

Algorithms have permeated throughout civil government and society, where they are being used to make high-stakes decisions about human lives. In this paper, we first develop a cohesive framework of algorithmic decision-making adapted for the public sector (ADMAPS) that reflects the complex socio-technical interactions between \textit{human discretion}, \textit{bureaucratic processes}, and \textit{algorithmic decision-making} by synthesizing disparate bodies of work in the fields of Human-Computer Interaction (HCI), Science and Technology Studies (STS), and Public Administration (PA). We then applied the ADMAPS framework to conduct a qualitative analysis of an in-depth, eight-month ethnographic case study of the algorithms in daily use within a child-welfare agency that serves approximately 900 families and 1300 children in the mid-western United States. Overall, we found there is a need to focus on strength-based algorithmic outcomes centered in social ecological frameworks. In addition, algorithmic systems need to support existing bureaucratic processes and augment human discretion, rather than replace it. Finally, collective buy-in in algorithmic systems requires trust in the target outcomes at both the practitioner and bureaucratic levels. As a result of our study, we propose guidelines for the design of high-stakes algorithmic decision-making tools in the child-welfare system, and more generally, in the public sector. We empirically validate the theoretically derived ADMAPS framework to demonstrate how it can be useful for systematically making pragmatic decisions about the design of algorithms for the public sector.

==> CWS Daily Algorithmic Practices 5.0 Camera Ready (ARXIV)/Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> CWS Daily Algorithmic Practices 5.0 Camera Ready (ARXIV)/RQ2table.tex <==
%============================== RQ2 =======================================
\begin{table}[]
\Small
\begin{center}
\begin{tabular}{|>{\raggedright}p{3cm}|>{\raggedright}p{5cm}|>{\raggedright\arraybackslash}p{5cm}|}
\hline
\rule{0pt}{1.3em}\cellcolor{mygray3}{\textbf{Framework Dimension}} & \rule{0pt}{1.2em}\cellcolor{mygray3}{\textbf{Positive Exemplar}} & \rule{0pt}{1.2em}\cellcolor{mygray3}{\textbf{Negative Exemplar}}\\
\hline
\multicolumn{3}{|l|}{\rule{0pt}{1.1em}{\textbf{Human Discretion}}}  \\
\hline
Professional Expertise  & \textit{} & \textit{"CANS has become all about the rate with little attention paid to actually helping the child"}\\
\arrayrulecolor{mygray2}\hline
Value Judgments   & \textit{} & \textit{"Caseworkers feel pressured to rate CANS higher to produce a higher compensation for foster parents"}\\
\arrayrulecolor{mygray2}\hline
Heuristic Decision-Making    & \textit{"Every case is different.. with 7ei we can focus on what's important for each case whether it's focusing on a child's trauma or parents' caregiver capacity"} &\\
\arrayrulecolor{black}\hline
\multicolumn{3}{|l|}{\rule{0pt}{1.1em}{\textbf{Algorithmic Decision-Making}}} \\
\hline
Relevant Data    & \textit{} & \textit{"CANS is frustrating because it lacks context about what’s going on with the child. It doesn’t account for the social structures that the kid interacts in."}\\
\arrayrulecolor{mygray2}\hline
Type of Decision-Support    & \textit{} & \textit{"Rate is generated by itself after we put in the CANS scores"}\\
\arrayrulecolor{mygray2}\hline
Degree of Uncertainty & \textit{""} & \textit{""}\\
\arrayrulecolor{black}\hline
\multicolumn{3}{|l|}{\rule{0pt}{1.1em}{\textbf{Bureaucratic Processes}}} \\
\hline
Resources \& Constraints  & & \\
\arrayrulecolor{mygray2}\hline
Admin. \& Training  & \textit{} &\\
\arrayrulecolor{mygray2}\hline
Laws \& Policies    & \textit{} &\\
\arrayrulecolor{black}\hline

\end{tabular}
\end{center}
\caption{RQ2: Balancing dimensions of framework}
\vspace{-0.3cm}
\end{table}
%============================== RQ2 =======================================

==> CWS Daily Algorithmic Practices 5.0 Camera Ready (ARXIV)/RQ3table.tex <==
%============================== RQ3 =======================================
\begin{table}[]
\Small
\begin{tabular}{|>{\raggedright}p{5cm}|>{\raggedright}p{6cm}|>{\raggedright\arraybackslash}p{2cm}|}
\hline
\rule{0pt}{1.3em}\cellcolor{mygray3}{\textbf{Theme}} & \rule{0pt}{1.2em}\cellcolor{mygray3}{\textbf{Illustrative Quotation}} & \rule{0pt}{1.2em}\cellcolor{mygray3}{\textbf{Codes}} \\
\hline
\multicolumn{3}{|c|}{\rule{0pt}{1.1em}{\textbf{Algorithmic decision-making should seek to augment human discretion rather than attempt to replace it 
}}}  \\
\hline
When aligned, algorithms augments decision-making processes, but a lack of alignment can takeaway autonomy and heuristic decision-making (85\%, n=17) & \textit{"7ei is embedded in the agency. Everything is based in the trauma-responsive model and often caseworkers are working through 7ei domains without even realizing it"} & values, heuristics, autonomy, discretion\\
\arrayrulecolor{mygray2}\hline
When aligned, algorithms can help embed important value judgments into the decision-making process (65\%, n=13) & \textit{"It [7ei] allows us to look at the case from the child's perspective and not just our own perspective. We might not trust mom but the child adores her. So we need to work with her and build that relationship"} & negotiate values, balance needs, personalized care\\
\arrayrulecolor{mygray2}\hline
Algorithms replacing the need for caseworker expertise can lead to inadequate and unreliable decision-making (70\%, n=14)
    & \textit{"We are reporting cases to HART just based on some risk factors on a checklist [AST]. It's not the full picture and only frustrates HART"} & lack of heuristics, high pressure, futile services\\
\arrayrulecolor{black}\hline
\multicolumn{3}{|l|}{\rule{0pt}{1.1em}{\textbf{Algorithmic decision-support systems and bureaucratic processes need to be aligned
}}} \\
\hline
When algorithmic decision-making and bureaucratic processes are aligned, it can help train caseworkers  (70\%, n=14)
  & \textit{"Every case is centered in the trauma-responsive model using 7ei. It ensures that caseworkers are always thinking through TIC"} & team expertise, supervision, engagement\\
\arrayrulecolor{mygray2}\hline
When the algorithmic decision-support system is not aligned with the constraints of the bureaucratic system, it leads to utility issues  (80\%, n=16)
   & \textit{"There are restrictions on how it [LPS] is used. You can’t rate a placement to be 'Good’ because you don’t have a court date set. But the hearing can go either way. We don't control that"} & time pressure, data fidelity, gaming the tool\\
\arrayrulecolor{mygray2}\hline
If the algorithms are not explained well to the professionals, they don’t trust them (70\%, n=14)
 & \textit{"[LPS] It's all perspective. Different people can be looking at the same issues, and have different reasons for saying the placement is 'good' or 'poor'"} & implicit use, hard to locate, other meanings\\
\arrayrulecolor{black}\hline
\multicolumn{3}{|l|}{\rule{0pt}{1.1em}{\textbf{Collective buy-in requires trust in algorithmic outcomes at both the caseworker and bureaucratic levels
}}} \\
\hline
When the algorithms miss important context, people don’t trust them (70\%, n=14)
  & \textit{"CANS does not account for underlying trauma or a child's support system.. which is essential"} & trauma, reductive, relationships\\
\arrayrulecolor{mygray2}\hline
There is collective buy-in when people feel like it leads to better outcomes (85\%, n=17)
 & \textit{"7ei scores show that trauma-informed meetings are actually leading to better placement stability and permanency outcomes"} & TIC practice, better outcomes, value-centered\\
\arrayrulecolor{mygray2}\hline
Lack of trust in algorithmic outcomes, leads to concerns about unethical and unsound decision-making (80\%, n=16)
   & \textit{"If several behaviors are scored high on CANS then that is a clear indicator that the caseworker was only trying to generate a higher rate"} & manipulate outcomes, lack of progress\\
\arrayrulecolor{black}\hline

\end{tabular}
\caption{RQ3: Benefits and Drawbacks of balancing Human Discretion, Algorithmic Decision-Making, and Bureaucratic Processes}
\label{RQ3:codebook}
\vspace{-0.8cm}
\end{table}
%============================== RQ3 =======================================

==> CWS Daily Algorithmic Practices 5.0 Camera Ready (ARXIV)/arrowTable.tex <==

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[]
\Small
\begin{tabular}{@{}|l|ll|ll|ll|@{}}
\toprule
                       & \multicolumn{2}{c|}{\textbf{Human Discretion}}                                                                                                               & \multicolumn{2}{c|}{\textbf{Algorithmic Decision-Making}}                                                                                                                                                                     & \multicolumn{2}{c|}{\textbf{Bureaucratic Processes}}                                                                                                                                                                          \\ \midrule
                       & \cellcolor[HTML]{FFE0D2}Professional Expertise    & \cellcolor[HTML]{FFE0D2}80\% \textcolor{red}{\faArrowDown}   & \cellcolor[HTML]{FFE0D2}Relevant Data         & \cellcolor[HTML]{FFE0D2}70\% \textcolor{red}{\faArrowDown}                                                                        & \cellcolor[HTML]{FFECB3}Resources/Constraints & \cellcolor[HTML]{FFECB3}40\% \textcolor{mygreen}{\faArrowUp} 70\% \textcolor{red}{\faArrowDown} \\
                       & \cellcolor[HTML]{FFE0D2}Value Judgments           & \cellcolor[HTML]{FFE0D2}75\% \textcolor{red}{\faArrowDown}   & \cellcolor[HTML]{FFE0D2}Decision-Support      & \cellcolor[HTML]{FFE0D2}90\% \textcolor{red}{\faArrowDown}                                                                        & \cellcolor[HTML]{FFECB3}Admin \& Training     & \cellcolor[HTML]{FFECB3}40\% \textcolor{mygreen}{\faArrowUp} 80\% \textcolor{red}{\faArrowDown} \\
\multirow{-3}{*}{\textbf{CANS}} & \cellcolor[HTML]{FFE0D2}Heuristic Decisions & \cellcolor[HTML]{FFE0D2}80\% \textcolor{red}{\faArrowDown}   & \cellcolor[HTML]{FFE0D2}Uncertainty & \cellcolor[HTML]{FFE0D2}70\% \textcolor{red}{\faArrowDown}                                                                        & \cellcolor[HTML]{DEF3D0}Laws \& Policies      & \cellcolor[HTML]{DEF3D0}80\% \textcolor{mygreen}{\faArrowUp}                                                                      \\
\hline
                       & \cellcolor[HTML]{DEF3D0}Professional Expertise    & \cellcolor[HTML]{DEF3D0}85\% \textcolor{mygreen}{\faArrowUp} & \cellcolor[HTML]{DEF3D0}Relevant Data         & \cellcolor[HTML]{DEF3D0}90\% \textcolor{mygreen}{\faArrowUp}                                                                      & \cellcolor[HTML]{DEF3D0}Resources/Constraints & \cellcolor[HTML]{DEF3D0}60\% \textcolor{mygreen}{\faArrowUp}                                                                      \\
                       & \cellcolor[HTML]{DEF3D0}Value Judgments           & \cellcolor[HTML]{DEF3D0}70\% \textcolor{mygreen}{\faArrowUp} & \cellcolor[HTML]{DEF3D0}Decision-Support      & \cellcolor[HTML]{DEF3D0}85\% \textcolor{mygreen}{\faArrowUp}                                                                      & \cellcolor[HTML]{FFECB3}Admin \& Training     & \cellcolor[HTML]{FFECB3}75\% \textcolor{mygreen}{\faArrowUp} 55\% \textcolor{red}{\faArrowDown} \\
\multirow{-3}{*}{\textbf{7ei}}  & \cellcolor[HTML]{DEF3D0}Heuristic Decisions & \cellcolor[HTML]{DEF3D0}85\% \textcolor{mygreen}{\faArrowUp} & \cellcolor[HTML]{DEF3D0}Uncertainty & \cellcolor[HTML]{DEF3D0}80\% \textcolor{mygreen}{\faArrowUp}                                                                      & \cellcolor[HTML]{FFE0D2}Laws \& Policies      & \cellcolor[HTML]{FFE0D2}65\% \textcolor{red}{\faArrowDown}                                                                        \\
\hline
                       & \cellcolor[HTML]{DEF3D0}Professional Expertise    & \cellcolor[HTML]{DEF3D0}70\% \textcolor{mygreen}{\faArrowUp} & \cellcolor[HTML]{FFECB3}Relevant Data         & \cellcolor[HTML]{FFECB3}65\% \textcolor{mygreen}{\faArrowUp} 75\% \textcolor{red}{\faArrowDown} & \cellcolor[HTML]{FFE0D2}Resources/Constraints & \cellcolor[HTML]{FFE0D2}60\% \textcolor{red}{\faArrowDown}                                                                        \\
                       & \cellcolor[HTML]{FFE0D2}Value Judgments           & \cellcolor[HTML]{FFE0D2}75\% \textcolor{red}{\faArrowDown}   & \cellcolor[HTML]{FFE0D2}Decision-Support      & \cellcolor[HTML]{FFE0D2}75\% \textcolor{red}{\faArrowDown}                                                                        & \cellcolor[HTML]{FFECB3}Admin \& Training     & \cellcolor[HTML]{FFECB3}65\% \textcolor{mygreen}{\faArrowUp} 60\% \textcolor{red}{\faArrowDown} \\
\multirow{-3}{*}{\textbf{AST}}  & \cellcolor[HTML]{FFE0D2}Heuristic Decisions & \cellcolor[HTML]{FFE0D2}75\% \textcolor{red}{\faArrowDown}   & \cellcolor[HTML]{FFE0D2}Uncertainty & \cellcolor[HTML]{FFE0D2}75\% \textcolor{red}{\faArrowDown}                                                                        & \cellcolor[HTML]{DEF3D0}Laws \& Policies      & \cellcolor[HTML]{DEF3D0}60\% \textcolor{mygreen}{\faArrowUp}                                                                      \\
\hline
                       & \cellcolor[HTML]{DEF3D0}Professional Expertise    & \cellcolor[HTML]{DEF3D0}40\% \textcolor{mygreen}{\faArrowUp} & \cellcolor[HTML]{FFE0D2}Relevant Data         & \cellcolor[HTML]{FFE0D2}65\% \textcolor{red}{\faArrowDown}                                                                        & \cellcolor[HTML]{FFE0D2}Resources/Constraints & \cellcolor[HTML]{FFE0D2}65\% \textcolor{red}{\faArrowDown}                                                                        \\
                       & \cellcolor[HTML]{FFE0D2}Value Judgments           & \cellcolor[HTML]{FFE0D2}60\% \textcolor{red}{\faArrowDown}   & \cellcolor[HTML]{FFE0D2}Decision-Support      & \cellcolor[HTML]{FFE0D2}60\% \textcolor{red}{\faArrowDown}                                                                         & \cellcolor[HTML]{FFE0D2}Admin \& Training     & \cellcolor[HTML]{FFE0D2}80\% \textcolor{red}{\faArrowDown}                                                                        \\
\multirow{-3}{*}{\textbf{LPS}}  & \cellcolor[HTML]{FFE0D2}Heuristic Decisions & \cellcolor[HTML]{FFE0D2}60\% \textcolor{red}{\faArrowDown}   & \cellcolor[HTML]{FFE0D2}Uncertainty & \cellcolor[HTML]{FFE0D2}65\% \textcolor{red}{\faArrowDown}                                                                        & \cellcolor[HTML]{DEF3D0}Laws \& Policies      & \cellcolor[HTML]{DEF3D0}65\% \textcolor{mygreen}{\faArrowUp}                                                                      \\ \bottomrule%\cmidrule(l){1-7} 
\end{tabular}
\vspace{0.1cm}
\caption{RQ3: Tradeoffs between balancing the dimensions within human discretion, algorithmic decision-making, and bureaucratic processes, Percentages (\%) represent the proportion of participants who stated that a dimension was positively (or negatively) impacted by the algorithm.} 
\vspace{-0.6cm}
\label{RQ3:arrowtable}
\end{table}

==> CWS Daily Algorithmic Practices 5.0 Camera Ready (ARXIV)/newResults.tex <==
\section{RESULTS}
In the following sections, we organize and present the results by our three research questions. First, we identify the high-stakes outcomes for which algorithmic decision-making is leveraged within CWS (RQ1) and the roles that human discretion, bureaucratic processes, and algorithmic decision-making play in these decision outcomes (RQ2). We do this separately for CANS, 7ei, AST, and LPS. Next, we discuss the potential benefits and drawbacks when balancing the different dimensions of ADMAPS framework (RQ3). Interviewees profiles can be found in the appendix.   

\subsection{{Child and Adolescent Needs and Strengths (CANS) Algorithm}}
The Child and Adolescent Needs and Strengths (CANS) algorithm was used at all the planning meetings (n=15) and discussed by all the interviewees (n=20). CANS algorithm is constructed using the CANS assessment; a communimetric tool designed to assess the level of need of a foster child and develop an individualized service plan \cite{lyons2004measurement}. With its primary purpose being communication, CANS assessment is designed based on communication theory rather than psychometric theories centered in measurement development \cite{lyons2009communimetrics}. CANS assessment was designed to support decision-making with respect to assessing a child’s level of need and service planning. However, as depicted in Figure \ref{fig:CANSoutcomes}, CANS algorithm has been re-appropriated to measure additional outcomes discussed below. It is conducted within the first 30 days of a child entering the child-welfare system or moving to a new placement (for e.g., foster home). It is then periodically conducted every six months.

%That is, the communimetric tool is not designed to explicitly measure any variables and only offers the child-welfare team a structured way to assess a case and share this information with other parties. However, the CANS algorithm has been re-purposed to measure the outcomes discussed below.  

\subsubsection{CANS High-Stakes Decision Outcomes (RQ1)} \leavevmode

\vspace{0.1cm}
\textbf{Mental Health Assessment and Level of Foster Care.}
All child-welfare workers at the agency are certified in conducting CANS for mental health screenings. As such, several participants (60\%, n=12) shared that the agency uses CANS algorithm to conduct a mental health assessment of foster children based on risks posed and exhibited behaviors. Participants (60\%, n=12) stated that the first CANS assessment was most useful because it helped establish a baseline for the mental-health needs of a child and the level of care that the child needed. For instance, one supervisor explained:

\begin{myquote}
    \textcolor{mygray}{\textit{"We need to have starting point.. what kind of behavioral issues does a child have? What are their needs? Because we can’t naively place a high-needs kid with foster parents who are not trained and certified to manage those needs. It’s a recipe for disaster"} -P9, Child Welfare Supervisor, MSW, 13 years}
\end{myquote}

The first assessment is used to devise service plans for foster children (for e.g, behavioral therapy) based on exhibited behaviors. It also facilitates sharing this information with other parties such as legal parties and family preservation specialists who also play a role in case planning. Child-welfare teams in both the planning meetings (n=15) and permanency consultations (n=40) briefly discussed child needs and behaviors but then shifted to a more extensive conversation about trauma using trauma-informed care. Some participants (50\%, n=10) also shared that CANS algorithm recommends the level of foster care that the child should be placed in (see Figure \ref{fig:CANSoutcomes}). Higher level foster homes are trained and certified in taking care of high-needs children. However, due to a lack of such homes, this decision often comes down to the availability of resources. 

\vspace{0.1cm}
\textbf{Compensation Calculations.} Using the CANS algorithm for calculating foster parents’ compensation was another prominent theme that emerged in 73\% (n=11) of the planning meetings and 85\% (n=17) of the interviews. However, it was not a dominant theme at the permanency consultations, because compensation is directly negotiated between the foster parents, case managers, and the supervisor. It does not require the input of rest of the child-welfare team. The state reimburses foster parents for the costs associated with having foster children placed in their homes. Most of the participants (85\%, n=17) quickly recognized CANS as the ``rate-setting tool'' even though compensation calculation was not the primary purpose of the algorithm. One supervisor explained:

\begin{figure}[t!]
  \includegraphics[scale=0.22]{CANSIMG.png}
  \caption{CANS Algorithm: Associated Decision Outcomes}
  \vspace{-0.2cm}
  \label{fig:CANSoutcomes}
  \vspace{-0.2cm}
\end{figure}

\begin{myquote}
    \textcolor{mygray}{\textit{"Foster parents who are taking in high-needs kids should be compensated for that. They have to put in significantly more time and energy in managing those behaviors, taking kids to therapy, setting healthy boundaries.. So we need this [CANS] standard to do that"} - P12, Child Welfare Supervisor, MSW, 7 years}
\end{myquote}

The state needs a \textit{metric} to be able to determine the compensation to be offered to each foster parent. The Department of Children and Families (DCF) decided to associate this compensation with the mental health needs of a child, that is, the higher the mental needs of a child, the higher the compensation offered to foster parents. Thus, even though the primary purpose of CANS was for conducting mental health assessments and for the level of foster care, it was re-appropriated to also calculate compensation associated with caring for a foster child's mental health needs. While it logically follows that a child with more mental health issues will require a higher level of care (consequently, higher cost of care), CWS employees were also well-aware that such cost-benefit analyses tied directly to something as subjective as mental health assessments were problematic.

\subsubsection{CANS and Algorithmic Decision-Making (RQ2)} 
Overall, caseworkers were frustrated that CANS misses important context about the child but is still used in a mandated predictive capacity. In the sections below, we discuss how CANS algorithm maps onto the dimensions of algorithmic decision-making (i.e., relevant data, type of decision-support, and degree of uncertainty). We use a percentage combined with an up or down arrow to denote the percentage of participants who indicated a positive or negative impact on each dimension of the ADMAPS framework for algorithmic decision-making, human discretion, and bureaucratic processes, respectively. We follow this structure throughout the remainder of our results. 

\vspace{0.1cm}
70\% \textcolor{red}{\faArrowDown} \textbf{Relevant Data.} \textit{CANS data does not account for trauma or social interactions}. Most of the participants (70\%, n=14) shared that CANS conducted the child’s assessment in an isolated manner and did not account for the quality and impact of relationships in their lives which are often more important for determining the long-term well being of these children. CANS algorithm focuses on the child emotional/behavioral needs (for e.g., anxiety, anger control, substance use, behavioral regression) and child risk behaviors (for e.g., suicide risk, self-harm, delinquent behavior, runaway tendencies) to assess the mental health needs of the child. For instance, a supervisor shared –

\begin{myquote}
    \textcolor{mygray}{\textit{"How do you measure empathy of others? You cant. Some foster parents are more empathetic and understanding and stand by the child no matter what. Sometimes that’s all it takes. You can’t put that in CANS"} -P15, Child Welfare Supervisor, 9 years}
\end{myquote}

Moreover, participants noted that CANS focuses on current behaviors but not the underlying trauma or traumatic triggers. The assessment is conducted based on exhibited behaviors over the past 30 days, however, the participants explained that trauma can stay with a child for years and lead to serious emotional dysregulation from time to time.

\vspace{0.1cm}
90\% \textcolor{red}{\faArrowDown} \textbf{Type of Decision-Support.}  \textit{The predictive nature of CANS leaves no room for discretion}. This challenge emerged in 90\% (n=18) of the interviews and 73\% (n=11) of the planning meetings. CANS algorithm is designed to predict or measure outcomes of interest once the data has been provided. Participants shared that the predictive nature of CANS leaves little room to exercise discretion and has become a great source of frustration for them. Gaming the inputs to achieve the desired outcome is the only way through which caseworkers regain agency. Participants explained that the higher the mental health needs of a child per CANS, higher the compensation offered to foster parents. After CANS scores are entered in, the algorithm generates a monetary value to be offered to foster parents. However, if foster parents disagree with the rate and believe they should be paid more, the caseworkers manipulate the scores to produce a higher rate. Most of the participants (90\%, n=18) shared their frustration regarding the inflexible and predictive nature of CANS. For instance, one supervisor explained:

\begin{myquote}
    \textcolor{mygray}{\textit{"Case managers and even supervisors are being forced to.. and kind of pressured into scoring children higher in order to provide higher numbers. So foster parents get paid more. CANS is a manipulative tool being used to barter off children...Children are being exploited for payment"} -P10, Child Welfare Supervisor, MS, LPC, NCC, 9 years}
\end{myquote}

\vspace{0.1cm}
70\% \textcolor{red}{\faArrowDown} \textbf{Degree of Uncertainty.} \textit{High degree of uncertainty associated with the outcomes}. Several participants (70\%, n=14) shared that CANS does not account for much of the data that they consider pertinent when assessing cases (for e.g., understanding about trauma and social support-system). This lack of relevant data leads to a high degree of uncertainty which is further exacerbated by the predictive and inflexible nature of CANS. Many felt that gaming the algorithm was the only viable option for caseworkers to exercise discretion. For instance, one supervisor shared:

\begin{myquote}
    \textcolor{mygray}{\textit{"CANS has become all about the rate. Generating the right rate so foster parents are happy with little to no attention paid to mental health needs"} -P13, Child Welfare Supervisor, MSW}
\end{myquote}

%===========================================================

\subsubsection{CANS Severely Impedes Human Discretion (RQ2).} In this section, we discuss how CANS algorithm maps onto the ADMAPS dimensions of human discretion. 

%-----------------------------------------------------------
\vspace{0.1cm}
80\% \textcolor{red}{\faArrowDown} \textbf{Professional Expertise.} \textit{CANS contradicts professional expertise}. All caseworkers at the agency are required to pass the CANS certification to be able to conduct the assessment with clients. However, most participants (80\% n=18) shared that their training in trauma-informed care (see Section 6.3), which offers a more comprehensive understanding of trauma and the child’s environment often conflicted with CANS. CANS further inhibited professional expertise because caseworkers felt that it turned them into data brokers who must collect information about children and feed it to the algorithm to make the decisions. The lack of relevant data and lack of decision-making latitude on part of caseworkers has turned CANS into primarily a rate-setting tool to calculate compensations. For instance, one case manager shared:

\begin{myquote}
    \textcolor{mygray}{\textit{"Caseworkers are doing CANS just to get it done.. to produce a good rate and reduce the conflict with foster parents. There is little to no attention paid to the mental health needs of kids."} -P17, Ongoing Case Manager, 8 years}
\end{myquote}

75\% \textcolor{red}{\faArrowDown} \textbf{Value Judgments.} \textit{CANS has introduced conflicting values}. Most of the participants (75\%, n=17) shared how the re-appropriation of CANS to calculate the foster parent compensations has led to several unintended consequences. CANS is re-conducted every six months to reassess the mental health needs of children, and consequentially, compensation is recalculated. However, with a focus on exhibited behaviors and not the underlying trauma, foster parents who are helping children cope and recover can see their compensation being lowered. A supervisor explained:

\begin{myquote}
    \textcolor{mygray}{\textit{"It is the complete opposite of what we want it [CANS] to do. Foster parents help minimize the behaviors and offer support so that kids can develop good coping skills. They help address the mental health needs and help kids stabilize by taking them to therapy and all their activities. But then they’re punished because the kid’s needs go down, and so does the rate"} -P9, Child Welfare Supervisor, MSW, 13 years}
\end{myquote}

Here, caseworkers are unable to prioritize properly conducting CANS because generating the adequate rate takes precedence to ensure the placement is not disrupted. Placement disruptions adversely affect foster children who develop emotional and behavioral problems and are unable to form lasting meaningful relationships with foster parents \cite{blakey2012review}. Therefore, caseworkers must prioritize supporting the current placement by any means necessary. This contradictory nature of CANS has turned caseworkers into value mediators and has left them frustrated because they are unable to adequately balance the needs of families and the demands of policymakers.

%-----------------------------------------------------------
\vspace{0.2cm}
80\% \textcolor{red}{\faArrowDown} \textbf{Heuristic Decision-Making.} \textit{CANS leaves no room for heuristic judgment calls}. This theme emerged in 80\% (n=16) of the interviews and 73\% (n=11) of the planning meetings. With a lack of relevant information pertinent to a case and high degree of uncertainty, it becomes imperative that caseworkers are able to turn towards heuristics and make decisions with the assistance of the child-welfare team. However, CANS does not allow for heuristic decision-making with respect to the outcomes. Participants (80\%, n=16) shared that every case is contextually different with salient factors that might be central to one case but peripheral to another. This was also apparent in all the planning meetings and permanency consultations where the teams adaptively focused on information pertinent to that case.

%===========================================================
\vspace{0.1cm}
\subsubsection{CANS and Bureaucratic Processes (RQ2).} Overall, CANS allocates resources but does not account for organizational constraints. In this section, we discuss how CANS algorithm maps onto the ADMAPS dimensions of bureaucratic processes.

\vspace{0.1cm}
40\% \textcolor{mygreen}{\faArrowUp} 70\% \textcolor{red}{\faArrowDown} \textbf{Resources \& Constraints.} \textit{CANS has introduced new constraints in the case planning process}. There is both a benefit and drawback to how CANS algorithm accounts for resources and constraints. Some participants (40\%, n=8) found value in the first assessment since it established the baseline for mental health and compensation for foster parents. Ideally, the algorithm offers an efficient way to allocate funds to foster parents based on mental health needs of the child. However, it does not account for organizational constraints and its implementation ends up introducing more constraints that frustrate caseworkers. Participants (70\%, n=14) shared that properly conducting CANS requires the caseworkers to interview several people, however, they are only able to interview foster parents due to high caseloads. A permanency consultant asserted:

\begin{myquote}
    \textcolor{mygray}{\textit{"You are supposed to interview foster parents and teachers as well as others that kids interact with to get a good CANS assessment. But with high caseloads, caseworkers only talk to the foster parents"} -P4, Permanency Consultant, MSW, APSW, 8 years}
\end{myquote}

However, as previously discussed, CANS is conducted every six months and foster parents are motivated to exaggerate behaviors to continue to be paid consistently. This is a constraint introduced by the implementation of the algorithm itself. Participants (50\%, n=10) also shared that the algorithm recommends the level of foster care that a child should be placed in, however, there is a lack of good foster homes in the system and this requirement is seldom met. Moreover, two data specialists shared that the caseworkers’ yearly job performance is tied to the timeliness with which they complete and submit CANS assessments since funds need to be allocated in a timely manner. Therefore, it exacerbates the need to get the assessments completed irrespective of the mental health needs of a child, and consequentially, adds another organizational constraint. 

\vspace{0.1cm}
40\% \textcolor{mygreen}{\faArrowUp} 80\% \textcolor{red}{\faArrowDown} \textbf{Administration \& Training.} \textit{Caseworkers are trained to conduct CANS but not on managing constraints}. This theme emerged in 80\% (n=16) of the interviews. CANS offers a way to support an organizational process of allocating resources. Caseworkers are trained and certified to conduct the mental health assessment, and as previously noted, some participants (40\%, n=8) found value in the first CANS assessment as a means to establish a baseline for mental health needs. However, they are not trained on how to manage the systemic constraints and value conflicts introduced by the algorithm itself. Participants (50\%, n=10) shared that new caseworkers socially learn from other caseworkers (and through experience) to manage these conflicts by gaming CANS. 

\vspace{0.1cm}
80\% \textcolor{mygreen}{\faArrowUp} \textbf{Laws \& Policies.} \textit{The use of CANS is legally mandated}. Most participants (80\%, n=18) recognized (and often complained) that CANS was legally mandated by the state and offered them a convenient means to allocate resources to foster parents every six months. Participants recognized that they must comply with this policy and continue implementing CANS enough though they routinely manipulated it to generate higher compensations.


%======================= 7ei algorithm =======================================
\subsection{Seven Essential Ingredients (7ei) Algorithm}
The agency uses trauma-informed care \cite{hendricks2011creating} as their core guiding principle, which is embedded in their practice and trauma-responsive service model \cite{topitzes2019trauma}. 7ei is a theoretically constructed algorithm that is centered in the medical practice of trauma-informed care (TIC) and complements the agency's social work practice \cite{hendricks2011creating, k2010shelter}. We witnessed 7ei being utilized in all meetings (N=55). This algorithm complements specialized trainings developed by the agency for child-welfare workers and introduces the complexity of trauma, frameworks for understanding the effects of trauma, and the practices and principles of TIC \cite{topitzes2019trauma}. 7ei acts as a guiding framework and is used to track and score each case from a TIC perspective. The algorithm is designed to be used in a team setting such that team members can offer their expertise, reach consensus decisions, and devise case plans. The team discusses and scores the child’s and caregiver’s wellness on seven domains as depicted in Figure \ref{fig:7eioutcomes} and brainstorms solutions on how to make progress on these domains. 7ei algorithm based in TIC has also been proven to improve child outcomes such as placement stability and permanence \cite{topitzes2019trauma}. 7ei assessments are individually focused, however, unlike CANS, the results are trauma-focused and also guide family interventions, highlighting areas of child functioning upon which the caregivers and professionals should focus their attention \cite{topitzes2019trauma}.

\begin{figure}[t!]
  \includegraphics[scale=0.25]{7eiIMG.png}
  \vspace{-0.6cm}
  \caption{7ei Algorithm: Associated Decision Outcomes}
  \vspace{-0.3cm}
  \label{fig:7eioutcomes}
\end{figure}


\subsubsection{7ei High-Stakes Decision Outcomes (RQ1)}
The seven domains of 7ei are: \textit{Prevalence}, \textit{Impact}, \textit{Perspective Shift}, \textit{Regulation}, \textit{Relationships}, \textit{Reasons to Be}, and \textit{Caregiver Capacity}. As such, 7ei is not directly tied to a specific outcome such that every time 7ei is used an outcome is recommended or predicted. Instead of predicting an outcome of interest using other factors, 7ei is used to track outcomes (i.e.- 7ei domains) over time to assess the trajectory of a child-welfare case. It is primarily used as a prescriptive tool that serves as a framework for team-based brainstorming of solutions guided by a TIC framework. As such, the seven domains of 7ei are both the input variables and the output variables of the 7ei assessment process because these are both the considerations and outcomes that the team is trying to measure and improve over time. Improvement in the 7ei domains is associated with placement stability and permanency outcomes, however, the agency leadership resisted developing a singular aggregate index that would measure this outcome. Ongoing conversations with agency leadership (program directors, quality improvement leaders) revealed that assessments are more likely to be manipulated if they are tied to singular metrics. Agency leadership also uses 7ei to assess progress within the agency with respect to trauma-informed care. For instance, it helps them understand whether conversations and meetings founded in TIC are leading to better permanency outcomes. Case-level outcomes of 7ei that are discussed at all the planning meetings and permanency consultations are depicted in Figure \ref{fig:7eioutcomes}.

\subsubsection{7ei and Algorithmic Decision-Making (RQ2)}
We found that the prescriptive nature of 7ei helps adaptively select data and address uncertainties. In this section, we discuss how 7ei algorithm maps onto the ADMAPS dimensions of algorithmic decision-making.

\vspace{0.1cm}
90\% \textcolor{mygreen}{\faArrowUp} \textbf{Relevant Data.} \textit{7ei provides a comprehensive view of the child and their ecosystem}. 
Participants shared that 7ei algorithm offers a comprehensive view of the foster child, caregivers, impact of traumatic events in their life, as well as interactions in their social ecosystem. Moreover, the child-welfare teams in all the permanency consultations (n=40) and planning meetings (n=15) were able to adaptively select factors that were most pertinent to that case. Most participants (90\%, n=18) emphasized that each case carried a lot of nuance and could not be addressed based on a few broad set of predictors so they appreciated that 7ei allowed them to focus on certain factors and then brainstorm ideas on how to help the family make progress. For instance, a program director shared:

\begin{myquote}
    \textcolor{mygray}{\textit{“We have tried the cookie cutter approach in the past. Assigning everyone to parenting classes, therapy, and other family support services. It failed and it is horrible to do to a family. So, with 7ei we focus on addressing core issues whether it’s the parent’s self-esteem, their own abandonment issues or child’s emotional regulation that will really help this family” } -P7, Child Welfare Program Director, MSW, 20 years}
\end{myquote}

Timeline of the case established which 7ei domains the child-welfare teams converged on. The teams focused more on some domains than others based on how long the child had been in the system. For instance, in case of children who had been in the system for a few months, the team spent more time on \textit{Prevalence} and \textit{Impact} and then focused on \textit{Perspective Shift} (see Figure \ref{fig:7eioutcomes}). Trauma symptoms are associated with negative short-term outcomes such as placement instability \cite{clark2020investigating}, therefore, the team focuses on recognizing trauma early on so that proper interventions could be made that promote healing and improving outcomes. However, cases that had been in the system for a longer period or had experienced multiple placement moves, the team focused more on \textit{Regulation}, \textit{Perspective Shift}, and \textit{Reasons to Be}. Prior studies show that placements are often disrupted because foster parents are unprepared to manage behaviors of traumatized children \cite{carnochan2013achieving, taylor2014perspectives}, therefore, the team focuses on these domains to assess how to improve self-regulation for the foster child as well as expand the caregivers’ understanding of trauma.

\vspace{0.1cm}
85\% \textcolor{mygreen}{\faArrowUp} \textbf{Type of Decision-Support.}  \textit{The prescriptive nature of 7ei allows for brainstorming and idea generation}. Most participants (85\%, n=17) appreciated that 7ei allowed for open discussions and brainstorming of solutions. 7ei is designed to be used in a team setting and acts as the TIC framework such that the child-welfare team deliberates over each domain, scores it, and formulates an action plan through a trauma-informed perspective. A case manager shared: 

\begin{myquote}
    \textcolor{mygray}{\textit{"I like 7ei because we use it as a team, and it allows us to brainstorm ideas. We look at not just the behaviors but the underlying trauma that is causing those behaviors."} -P18, Case Manager, BSW, 2 years}
\end{myquote}

The 7ei domains are also the outcomes of interest that the team seeks to track and affect over time. Improvements in these domains are directly associated with the outcomes of placement stability and permanency which are tracked at the agency level.

\vspace{0.1cm}
80\% \textcolor{mygreen}{\faArrowUp} \textbf{Degree of Uncertainty.}  \textit{Adaptively selecting relevant data helps address high degree of uncertainty}. Most participants (80\%, n=16) felt that every case was contextually different and required their individual attention. That is, it was imperative they adequately weigh nuances and factors pertinent to that case. 7ei allows the child-welfare team to adaptively select the domains pertinent to a case and spend significantly more time on them and brainstorm solutions. Tracking outcomes over time and not using the tool in a predictive capacity allows the team to mitigate the high degree of uncertainty that would otherwise be associated with the predictions. 

%------------------------------------------------------------------------------
\subsubsection{7ei Augments Human Discretion (RQ2).} In this section, we discuss how the 7ei algorithm maps onto the ADMAPS dimensions of human discretion.

%--------------------------%
\vspace{0.1cm}
85\% \textcolor{mygreen}{\faArrowUp} \textbf{Professional Expertise.} \textit{7ei helps develop professional expertise.} The algorithm is theoretically constructed and is centered in trauma-informed care. Participants (85\%, n=17) believed that it allowed them to brainstorm ideas from a TIC perspective and develop plans specific to that family. Continuous engagement with 7ei in trauma-informed meetings ensures that caseworkers are always thinking through TIC frameworks.  A permanency consultant asserted:

\begin{myquote}
    \textcolor{mygray}{\textit{"7ei isn’t just a "thing" that we do. It is centered in everything that we do. It ensures that caseworkers are always thinking through TIC frameworks"}  -P1, Permanency Consultation Supervisor, MSW, APSW, 22 years
}
\end{myquote}

This is especially important for CWS since the system lacks experienced caseworkers due to high turnover \cite{carnochan2013achieving}. Continually working through 7ei under proper supervision ensures that new caseworkers are developing professional expertise.

%-------------------------%
\vspace{0.1cm}
70\% \textcolor{mygreen}{\faArrowUp} \textbf{Value Judgments.} \textit{7ei allows caseworkers to make informed value judgments}. This theme emerged in 70\% (n=14) of the interviews and 72\% (n=40) of the meetings. 7ei is centered in social work’s core values of service, dignity, and worth of the person and allows caseworkers to prioritize these values and devise interventions that will directly help a child and their family cope with trauma. For instance, prioritizing the well-being of a child does not only mean sending them to therapy. It also incorporates addressing concerns within their ecosystem. A supervisor explained: 

\begin{myquote}
    \textcolor{mygray}{\textit{"Therapy only goes so far if nothing changes in the child’s ecosystem and they feel continually triggered by others. With 7ei we try to address problems in this ecosystem and devise approaches that will help the family"}  -P9, Child-Welfare Supervisor, 13 years
}
\end{myquote}

%"It [7ei] allows us to look at the case from the child's perspective and not just our own perspective. We might not trust mom but the child adores her. So we need to work with her and build that relationship"

7ei allows the child-welfare team to make value-based judgments and take steps that improve the quality of a child's relationships. This takes the form of family-level interventions or sharing information with caregivers about the impact of trauma to bring about a perspective shift.

%-------------------------%
\vspace{0.1cm}
85\% \textcolor{mygreen}{\faArrowUp} \textbf{Heuristic Decision-Making.} \textit{7ei enables heuristic judgment calls}. Most participants (85\%, n=17) appreciated that 7ei offered them flexibility and autonomy in how they interact with it. This theme also emerged in all the planning meeting (n=15) and permanency consultations (n=40) where the child-welfare team adaptively selected information that was most pertinent to the case and often acted as an obstacle towards achieving permanency. For instance, cases where the child had experienced multiple placement moves, the team focused on \textit{Regulation} and \textit{Reasons to Be} to devise plans that would help improve the child’s emotional, behavioral, and cognitive functioning. 

%Similarly, cases where a parent’s lack of caregiver capacity was the obstacle that prevented reunification, the team focused on plans that would help the parent develop caregiver capacity as well as utilize their own support system in the form of parents and relatives who could help with the children. 

\subsubsection{7ei Supports Bureaucratic Processes (RQ2).} In this section, we discuss how the 7ei algorithm maps onto the ADMAPS dimensions of bureaucratic processes.

\vspace{0.1cm}
60\% \textcolor{mygreen}{\faArrowUp} \textbf{Resources \& Constraints.} \textit{7ei accounts for the resources at the organization}. Participants (60\%, n=12) shared that 7ei is locally developed at the agency and accounts for the resources available at the agency in the form of supervision, expertise, and specialized trainings. Participants also shared that critical decision-making power in regard to achieving permanency sits with the legal parties (district attorneys, judges), however, 7ei operates within these constraints and allows caseworkers to help families and prepare them to be able to receive a favorable decision in court.

\vspace{0.1cm}
75\%\textcolor{mygreen}{\faArrowUp} 55\%\textcolor{red}{\faArrowDown}  \textbf{Administration \& Training.}  \textit{7ei is embedded in daily work processes but requires additional oversight and training}. This theme emerged in 75 \% (n=15) of the interviews and all the planning meetings (n=15) and permanency consultations (n=40) and there is both a benefit and a drawback associated with it. Participants (75\%, n=15) recognized that continually engaging with the tool in meetings was helpful but some participants (55\%, n=11) shared that the tool also added more tasks to an already heavy workload. The agency offers specialized trainings for trauma-informed care with 7ei acting as a tool that complements these trainings. Moreover, we observed that 7ei is embedded into daily work processes because it is utilized every time a case is discussed in a team setting. This continued engagement under supervision has helped earn the trust of caseworkers who learn not just from the algorithm but also the collective expertise of the child-welfare team. For instance, a case manager shared:

\begin{myquote}
    \textcolor{mygray}{\textit{"I like 7ei because we use it as a team, and it allows us to brainstorm ideas. It just helps.. thinking out loud with everyone and knowing that I don't have make these decisions alone. Also, it helps guide my thought process but doesn’t tell me what to do."} -P17, Case Manager, BSW, 8 years}
\end{myquote}

However, 7ei has added to the workload of both the case managers and supervisors who must discuss and complete an additional tool as part of their job requirement at the agency. 

\vspace{0.1cm}
65\% \textcolor{red}{\faArrowDown} \textbf{Laws \& Policies.} \textit{7ei is not legally mandated and only used locally at the agency}. Several participants (65\%, n=13) were frustrated by the fact that 7ei was not legally mandated and that they had to continue using CANS. Even though an independent research study showed that 7ei is leading to better permanency and placement outcomes, the algorithm still lacks legitimacy at the state and federal level. 

%========================Anti Sex-Trafficking Algorithm================================

\subsection{Anti Sex-Trafficking (AST) Algorithm}
An emerging high-stakes decision for which an algorithm is used is assessing the risk of sex-trafficking for a foster child over 10 years of age. We observed this in 65\% (n=13) of the interviews, 33\% (n=5) of the planning meetings, and 35\% (n=14) of the permanency consultations. The agency has a dedicated team called HART (Human Anti-Trafficking Response Team) that manages cases where the foster child might be at high risk of being trafficked. If a child meets the criteria for risk of sex-trafficking per the AST algorithm, the case must be reported to HART. Early identification of such indicators can play a significant role in ensuring child safety.

%It is a checklist-style screening algorithm that consists of several indicators that have been associated with sex-trafficking in the past. 

%Youth in the child-welfare system are at high risk of being victimized by sex-trafficking and the child-welfare agencies are increasingly becoming aware of these risks and developing mechanisms in terms of organizational processes to address these concerns. For instance, this

\subsubsection{AST High-Stakes Decision Outcomes (RQ1)} Risk indicators are divided into three domains - "At-Risk", "High-Risk", and "Confirmed". The child-welfare team must continue to closely monitor the case if they select fewer than three "At-Risk" indicators and continue to have conversations to mitigate the risks. If the team selects three or more "At-Risk" indicators or 1 or more "High-Risk" or "Confirmed" indicators, then the case must be referred to HART.

\subsubsection{AST and Algorithmic Decision-Making (RQ2)}
Overall, we found that AST algorithm often missed important context, which frustrated caseworkers. In this section, we discuss how AST algorithm maps onto the ADMAPS dimensions of algorithmic decision-making.

\vspace{0.1cm}
65\% \textcolor{mygreen}{\faArrowUp} 75\% \textcolor{red}{\faArrowDown} \textbf{Relevant Data.} \textit{AST assesses pertinent risk indicators but misses context about the case}. Several participants (65\%, n=13) shared that the algorithm offers a new perspective on sex-trafficking by capturing risk indicators that they had not considered before. For instance, “possession of money, electronics, cosmetics, or clothes that are unexplained”, “traveling out of the area or somewhere out of the ordinary”, and “unwilling to provide information about an older partner” are some of these indicators. A supervisor shared:

\begin{myquote}
    \textcolor{mygray}{\textit{"It’s helpful to have us think about it differently. I have been doing this for a very long time and when I started, we were never thinking about trafficking. So now we are more conscious of these risks" } -P8, Child Welfare Supervisor, MSW, APSW, 19 years}
\end{myquote}

However, participants (75\%, n=15) also shared that the algorithm misses context about each case and the presence of some of these risk indicators did not mean the child was being sex trafficked.

\vspace{0.1cm}
75\% \textcolor{red}{\faArrowDown} \textbf{Type of Decision-Support.} \textit{Predictive nature of AST frustrates caseworkers}. Several participants (75\%) who found value in the algorithm as a guide also shared their frustrations in regard to its mandatory reporting nature. AST is used in a predictive capacity such that if certain risk indicators are selected then the case must be reported to HART.  For instance, a permanency consultant shared:

\begin{myquote}
    \textcolor{mygray}{\textit{"If a child is at risk for sex trafficking then we are having those conversations from the very beginning and taking necessary action. This decision tool is not helpful in the way it’s being used and only frustrates HART"} -P5, Permanency Consultant. MSW, 12 years}
\end{myquote}
 
Reporting to HART takes the case away from the child-welfare team who have spent significant amount of time building a relationship with the child and their caregivers. Moreover, HART is receiving an influx of calls that do not require their expertise as a result of this algorithm.

\vspace{0.1cm}
75\% \textcolor{red}{\faArrowDown} \textbf{Degree of Uncertainty.} \textit{Lack of context about the case leads to high degree of uncertainty}. Several participants (75\%, n=15) shared that even though AST was useful as a guide, the presence of risk indicators did not mean the child was at risk of being trafficked. There was still a lot of pertinent information that was necessary to make such a determination. For instance, a supervisor shared that one of their foster kids had a history of sexual abuse and met a bunch of criteria on the tool, however, the supervisor’s team is actively involved with the child and their caregivers, understand their needs, and did not believe the case needed to be reported to HART.  

%----------------------------------------------------------%

\subsubsection{AST Impedes Human Discretion (RQ2)} In this section, we discuss how AST algorithm maps onto the ADMAPS dimensions of human discretion.

\vspace{0.1cm}
70\% \textcolor{mygreen}{\faArrowUp} \textbf{Professional Expertise.} \textit{AST has made caseworkers more aware of risk indicators}. Most participants (70\%, n=14) appreciated that this decision-tool taught new caseworkers to be actively aware of indicators that are associated with sex trafficking. As stated by P5 above, AST has improved professional expertise since caseworkers are more cognizant of such risks.

\vspace{0.1cm}
75\% \textcolor{red}{\faArrowDown} \textbf{Value Judgments and Heuristic Decision-Making.} \textit{AST does not allow caseworkers to make value judgments or engage in heuristic decision-making}. Several participants (75\%, n=15) shared that the risk indicators were just part of a bigger picture and there was still a lot context that the child-welfare team needed to collectively unpack to better assess the situation. This requires the child-welfare team to engage in heuristic decision-making and weigh the necessary information. For instance, a case manager shared:

\begin{myquote}
    \textcolor{mygray}{\textit{"One of my foster teens is sexually active and has a long-term boyfriend. But looking at the tool, everyone is like... ‘Is that her boyfriend or her pimp?’ I know this kid and she trusts me... building trust with these kids takes time... she doesn’t need to be referred to HART [Human Anti-Trafficking Response Team]"} -P17, Case Manager, BSW, 8 years}
\end{myquote}

Here, the case manager emphasizes that having trusting relationships was equally important for preventing foster youth from being sex trafficked. Referring the case to HART takes this case away from the case manager and the child is assigned a new case manager from HART.

%---------------------------------------------------
\subsubsection{AST and Bureaucratic Processes (RQ2)} Overall, we found that AST is inadequately supported by bureaucratic processes which leads to frustrations on part of caseworkers. In this section, we discuss how AST algorithm maps onto the ADMAPS dimensions of bureaucratic processes.

\vspace{0.1cm}
60\% \textcolor{red}{\faArrowDown} \textbf{Resources \& Constraints.} \textit{AST has caused an influx of cases referred to HART}. Several participants (60\%, n=12) shared that AST has added to the frustrations of HART who do not have enough resources to manage all the cases that are being reported to them because of the mandatory reporting aspect of AST. This leaves HART with significantly less resources to focus on the cases that need them. A supervisor on HART explained:

\begin{myquote}
    \textcolor{mygray}{\textit{“It's become overused and is being abused. It's being used in different settings and not how it was originally intended to be used. We are getting an influx of calls that don't need to be called.”} -P10, Child Welfare Supervisor, MSW, LPC, NCC, 9 years}
\end{myquote}

\vspace{0.1cm}
65\% \textcolor{mygreen}{\faArrowUp} 60\% \textcolor{red}{\faArrowDown} \textbf{Administration \& Training.} \textit{AST is conducted as an organizational process and offers some training}. Most participants (65\%, n=13) shared that AST is routinely conducted for foster youth over 10 years of age. As discussed previously, it trains new caseworkers to be more conscious about risk factors but often to the detriment of HART. Participants also consider this decision-tool to be peripheral to the case planning process for most cases and utilized it as a mandated requirement.

\vspace{0.1cm}
60\% \textcolor{mygreen}{\faArrowUp} \textbf{Laws \& Policies.} \textit{The use of AST is mandated by law}. The Department of Children and Families (DCF) has legally mandated the use of this algorithm as a means to proactively protect foster youth as well as collect more data about associated risk factors and the number of foster youth considered at risk. Next, we discuss the Legal Permanency Status (LPS) algorithm.

%===================== Legal Permanency Status (LPS) Algorithm ===============================
\subsection{Legal Permanency Status (LPS) Algorithm} Tracking performance metrics such as placement stability and permanency emerged as another decision outcome for which an algorithm is being used. Several participants (65\%, n=13) discussed this decision-tool, and we observed the tool being used at all the permanency consultations (n=40). Federal legislation has established permanency as one of the primary goals of CWS and requires agencies to meet this well-defined and measurable benchmark \cite{williams2014child}. Legal permanency is defined as reunification with the biological family, adoption or transfer of guardianship. \cite{koh2008propensity}. 
%This tool establishes a sense of urgency and insistence towards achieving permanency since prolonged instability and multiple placement moves leads to poor well-being outcomes for foster children. 

%------------------------------------------------------------------------
\subsubsection{LPS High-Stakes Decision Outcomes (RQ1)}
This algorithm is used to track an outcome over time instead of predicting an outcome of interest using input data. The agency uses it at permanency consultations to track the quality of the current placement and if those specialized meetings are leading to better outcomes. The tool is facilitated by the permanency consultant and upon completion, the team categorically rates the quality of the placement. It is also used to track systemic barriers that are getting in the way of achieving permanency. Some participants recognized (40\%, n=8) the utility of this tool and a permanency consultant explained – 

\begin{myquote}
    \textcolor{mygray}{\textit{"It helps us to be actively aware of where we are at in terms of permanency. We have to follow a [15-month] timeline for permanency and if parents are not showing initiative and not completing court ordered services then we need to start exploring placement options. So, this tool is kind of an extra push"} -P5, Permanency Consultant, MSW, 12 years}
\end{myquote}
 
%------------------------------------------------------------------------

\subsubsection{LPS and Algorithmic Decision-Making (RQ2)} Overall, we found that even though LPS is used in a prescriptive capacity, it still lacks utility. In this section, we discuss how LPS algorithm maps onto the ADMAPS dimensions of algorithmic decision-making.

\vspace{0.1cm}
65\% \textcolor{red}{\faArrowDown} \textbf{Relevant Data.} \textit{Definitions of input variables are ambiguous and frustrate caseworkers}. Several participants (65\%, n=13) shared their indifference towards LPS and stated that the definitions of input variables in terms of what constitutes a “Good”, “Fair”, or “Poor” placement were ambiguous. A permanency consultant who is tasked with conducting this decision-tool shared:

\begin{myquote}
    \textcolor{mygray}{\textit{“This tool is confusing in itself; the definitions are very vague. We can't necessarily put families into categories. We have to use this tool and have conversations about where they [families] might fit best, but it doesn’t give a clear picture of what's really going on with the placement.”} - P6, Permanency Consultant, BSW, 3 years}
\end{myquote}

Participants (65\%, n=13) also shared that how LPS was conducted depended on the perspective of the team. Different people might look at the same set of facts and reach different conclusions as to why the placement should be rated as good, fair, or poor. 

\vspace{0.1cm}
60\% \textcolor{red}{\faArrowDown} \textbf{Type of Decision-Support.} \textit{LPS is used as a prescriptive tool, but caseworkers lack agency towards affecting outcomes}. Participants (60\%, n=12) shared that the tool did not predict or recommend an outcome based on the inputs, however, the utility of the tool lies in recognizing the current state of a case with respect to permanency and addressing systemic barriers, but the child-welfare team lacks agency with respect to addressing several systemic barriers. For instance, critical decision-making power in regard to permanency decisions sits with the legal parties (district attorneys and judges) who can choose to fully disregard the child-welfare team’s recommendation. 

\vspace{0.1cm}
65\% \textcolor{red}{\faArrowDown} \textbf{Degree of Uncertainty.} \textit{Lack of relevant information leads to high degree of uncertainty}. Participants (65\%, n=13) were most frustrated by the lack of relevant information that LPS needed to account for in order to make a proper determination about the quality of the placement. Moreover, there is high uncertainty associated with the timeliness with which some systemic barriers can be addressed making it hard to assess the quality of the placement (see P2 quote below).

%------------------------------------------------------------------------
\subsubsection{LPS impedes Human Discretion (RQ2)} In this section, we discuss how LPS algorithm maps onto the ADMAPS dimensions of human discretion.

\vspace{0.1cm}
40\% \textcolor{mygreen}{\faArrowUp} \textbf{Professional Expertise.} \textit{LPS builds professional expertise by establishing an urgency towards permanency}. Some participants (40\%, n=8) shared that the decision-tool was useful in that it established a sense of urgency and insistence towards achieving permanency for foster children. It teaches new caseworkers that they needed to prioritize finding placement options even if that upset biological parents. The child-welfare team follows a 15-month timeline where the parents must complete court order services within this timeline to achieve reunification. Towards the end of this timeline, CWS team must begin exploring alternate placement options.

\vspace{0.1cm}
60\% \textcolor{red}{\faArrowDown} \textbf{Value judgments and Heuristic Decision-Making.} \textit{LPS tool does not allow for value judgments or heuristics}. Participants (60\%, n=12) shared that the tool does not allow for value judgments or heuristics on part of the child-welfare team since decision-making power about permanency decisions sits with the legal parties.

%------------------------------------------------------------------------
\subsubsection{LPS and Bureaucratic Processes (RQ2)} Overall, LPS supports bureaucratic processes but does not account for organizational constraints. In this section, we discuss how LPS algorithm maps onto the ADMAPS dimensions of bureaucratic processes.

\vspace{0.1cm}
65\% \textcolor{red}{\faArrowDown} \textbf{Resources \& Constraints.} \textit{LPS does not account for organizational resources and imposes new constraints}. Participants shared (65\%, n=13) that ambiguity around input variables and lack of agency with respect to permanency decisions has turned this decision-tool into documentation that every child-welfare team must complete at permanency consultations. Moreover, there are arbitrary constraints placed on the decision-tool in regard to how a placement can be rated. For instance, a program director explained:

\begin{myquote}
    \textcolor{mygray}{\textit{"We may have a court hearing date set and all of a sudden, the placement is “Good”. We now have a "Good" rating because we have a court hearing. But it might take three years to terminate parental rights or go to a guardianship. And then you went three years without achieving permanency but somehow, we have a “Good" placement rating."} -  P2, Permanency Consultant, MSW, 20 years}
\end{myquote}

\vspace{0.1cm}
80\% \textcolor{red}{\faArrowDown} \textbf{Administration \& Training.} \textit{Caseworkers are indifferent towards how LPS is administered}. Even though the tool is expected to be central to permanency consultations, we noticed that for majority of these meetings (87\%, n=35), LPS was used towards the end as a requirement to rate the quality of the placement. Most participants (80\%, n=16) were indifferent towards LPS because of the several constraints and utility issues discussed above. One supervisor shared:

\begin{myquote}
    \textcolor{mygray}{\textit{"It’s just another thing we have to do in the permanency meetings. I let the Permanency Consultants score it however they like"} - P15, Child Welfare Supervisor, MSW, 9 years}
\end{myquote}

\vspace{0.1cm}
65\% \textcolor{mygreen}{\faArrowUp} \textbf{Laws \& Policies.} \textit{The use of LPS tool is legally mandated and helps track performance outcomes}. Participants (65\%, n=13) shared that the Department of Children and Families (DCF) has mandated using this decision-tool as a way to track the important outcomes of quality of placements and permanency. Moreover, it’s important to track the systemic barriers that often impact permanency to formulate policies at the state level that address these systemic barriers.


%=======================TABLE TABLE ===========================================

% \begin{figure}
% \fontsize{7.8}{10}\selectfont
%   \includesvg[scale=0.90]{New Figures/tabley-6.svg}
%   \vspace{-0.3cm}
%   \caption{Tradeoffs between balancing the dimensions within human discretion, algorithmic decision-making, and bureaucratic processes}
%   \vspace{-0.2cm}
%   \label{fig:outcomes}
% \end{figure}

%=============================== RQ3 ==========================================

\subsection{Assessing the Benefits and Drawbacks of Differing Approaches (RQ3)}
 Table \ref{RQ3:arrowtable} offers a summary of how the four algorithms balance the dimensions of the framework. In this section, we discuss the benefits and drawbacks that arise when trying to balance the tradeoffs between human discretion, algorithmic decision-making, and bureaucratic processes.

\subsubsection{Algorithmic Decision-Making Should Seek to Augment Human Discretion, Not Supplant it.} In this section, we discuss the themes around the benefits and drawbacks that emerged when balancing the ADMAPS dimensions of human discretion and algorithmic decision-making.

\vspace{0.2cm}
\textbf{When aligned, algorithms augment decision-making processes, but a lack of alignment can take away autonomy and heuristic decision-making.} All of our participants emphasized that every case is contextually different and that a family’s circumstances often change through the life of the case. For instance, a parent seeking reunification with their child might experience a lapse while trying to maintain a stable job, maintain their sobriety, or consistently attend court ordered services. In other words, algorithms should be designed with the recognition that there will be a high degree of uncertainty associated with any relevant data and the subsequently predicted outcome. Therefore, algorithms need to not only make room for human discretion but also facilitate value judgments and heuristics in order to offer utility. Most of our participants (80\%, n=16) mentioned that 7ei algorithm augmented their decision-making processes when they were making difficult decisions. It prioritizes and enhances the value judgments and heuristic decision-making that caseworkers must engage in when devising action steps to help families. Participants (85\%, n=17) especially appreciated that 7ei facilitated brainstorming and idea generation instead of predicting an outcome of interest. One case manager explained:

\begin{myquote}
    \textcolor{mygray}{\textit{"Of all the things we have brought up, 7ei is my favorite because its helps us think differently, understand what a family has been through and then brainstorm ideas on how to help them based on this understanding of trauma"} -P3, Permanency Consultant, MSW, APSW, 9 years}
\end{myquote}

%In the permanency consultations, the child-welfare teams focused on the 7ei domains that required more attention than others. For instance, cases where \textit{the Reasons to Be} domain had been consistently scored low, the child-welfare team would discuss efforts towards building relationships and getting the child engaged in activities that may provide them with a sense of purpose and also offer them the opportunity to build new relationships.

Participants noted that the tool offers flexibility and autonomy in how they interact with it and which 7ei domains they focused on. Adaptively selecting information instead of analyzing all the information is a key feature of heuristic decision-making and can lead to more accurate decisions. On the other hand, tensions arise when algorithms attempts to supplant human discretion. This is the case with CANS whose predictive nature does not account for the high degree of uncertainty that accompanies each case, and consequently, does not make room for discretionary work on part of the caseworkers. With a lack of autonomy, gaming the algorithm is the only way caseworkers are able to exercise discretion and produce the desired outcome. One supervisor shared: 

\begin{myquote}
    \textcolor{mygray}{\textit{"CANS is all about producing a good rate so foster parents can afford the resources they need to take care of the child. I have had foster parents put in notices [to end placement] because they couldn't support the child anymore"} -P14, Child Welfare Supervisor, MSW, 30 years}
\end{myquote}

This inflexible and predictive nature has shifted focus away from the primary outcome of interest (i.e. – mental health screening) and towards the secondary outcome that allocates resources.

\input{arrowTable}

\vspace{0.2cm}
\textbf{When aligned, algorithms can help embed important value judgments into the decision-making process}. Most of the participants (80\%, n=16) felt strongly about the need to support each family in a different capacity and through different practices. This was also a dominant theme in all the planning meetings (n=15) and permanency consultations (n=40) where the child-welfare team devised specific plans for each family through trauma-informed care (i.e. - using 7ei). 7ei algorithm is centered in some of social work’s core values of service, dignity and worth of the person, and importance of human relationships \cite{topitzes2019trauma} and informs the child-welfare team’s work processes. For instance, a supervisor explained: 

\begin{myquote}
    \textcolor{mygray}{\textit{"7ei helps us think about how we can help every family. What can we do to help mom develop her self-worth? How can we help her build relationships with relatives or people in the community, so she has more caregiver support"} -P8, Child Welfare Supervisor, MSW, CAPSW, 19 years}
\end{myquote}

Several participants (65\%, n=13) explained that 7ei scores translated into actionable steps that directly sought to help children and their families. In the meetings, 7ei brainstorming sessions resulted in solutions that the child-welfare team could affect directly and not simply refer children and parents to therapy. For instance, the case managers and supervisors planned activities that the family could engage in to improve child as well as family functioning, discussed information to share with foster and biological parents about impacts of trauma exposure, as well as steps caregivers could take to establish healthy boundaries with foster children and enforce positive discipline. For instance, a permanency consultant explained:

\begin{myquote}
    \textcolor{mygray}{\textit{"It [7ei] helps you have a perspective shift on the family and the child. You don’t need to refer everyone and their mother to therapy. Sometimes it’s just as simple as having them do something as a family that’s different than what they ever did before [picnics, sports].. and challenge them in different ways"} -P2, Permanency Consultant, MSW, 20 years}
\end{myquote}

On the contrary, algorithms that do not embed human values into its design may consequentially end up minimizing them. For instance, CANS recommends the level of foster care that the child should be placed in and based on that the child-welfare team finds foster parents who have the resources to meet those needs. However, participants explained that more financial resources do not always equate to a foster child’s well-being. For instance, a permanency consultant explained: 

\begin{myquote}
    \textcolor{mygray}{\textit{"Everyone has a different compass for well-being. We had a child who was placed with well-off foster parents in a five-bedroom house and he wasn't doing well there because it was a culture shock for him. He wasn't used to a huge home, a great school, a big backyard... and he completely shut down. So, we found his aunt and we moved him down to Chicago. It's a two-bedroom house with five other kids and this child is thriving! So, he needed to be with his family, and he needed to have his own culture.} -P4, Permanency Consultant, MSW, APSW, 8 years}   
\end{myquote}

Here the permanency consultant emphasizes the core human value of having trusting relationships in one’s life and the importance of one’s culture that play a critical role towards achieve emotional and cognitive well-being. Unlike CANS, 7ei allowed the child-welfare team to prioritize \textit{Reasons To Be} and \textit{Regulation} to really help children instead of simply focusing on financial resources. Caseworkers must continually negotiate values and balance the individual needs of people with the demands of policymakers. Algorithms that do not allow caseworkers to make such value judgments may lead to more frustrations and limit their utility.

%We argue that frontline workers become moral mediators, tasked with interfacing between the individual needs of citizens and the demands of policymakers

\vspace{0.1cm}
\textbf{Algorithms that replace the need for caseworker expertise can lead to inadequate and unreliable decision-making}. Another dominant theme that emerged in 70\% (n=14) of the interviews, 53\% (n=8) of the planning meetings, and 50\% (n=20) of the permanency consultations was that the algorithms in use were diminishing the need for caseworker expertise and family-centered care in a very contextual domain. CWS is a high-stakes domain where most caseworkers lack adequate work experience, carry high caseloads, and are under a lot of pressure from legal parties. Most of the participants (70\%, n=14) expressed concerns that algorithmic systems might simply act as a safe default for most caseworkers such that questioning an algorithmic decision would add more work to their plate. A program director explained – 

\begin{myquote}
    \textcolor{mygray}{\textit{"We are not hiring people with a lot of experience. All new hires are recent graduates who don’t quite know what this field looks like. They are happy to trust the machine to just get through the day"} -P7, Child Welfare Program Director, MSW, 20 years}
\end{myquote}

Professional expertise in the public sector deteriorates when algorithms limit the scope for value judgments and heuristic decision-making. Value negotiations and heuristics are an indispensable aspect of professional practice that workers must continually engage in to build expertise \cite{loyens2010toward}. There are also growing concerns that algorithms such as CANS are leading to children being referred to unnecessary services which also shifts the focus away from family-centered care. CANS scores directly translate to actionable steps in the form of services that children are referred to. Caseworkers co-opt CANS to produce higher compensations for foster parents or the foster parents might exaggerate child behaviors, however, several participants (60\%, n=12) recognized that this also meant unnecessary services being requested for children. One case manager explained: 

\begin{myquote}
    \textcolor{mygray}{\textit{"Foster parent might exaggerate behaviors just to get more money. And then we put the kid in therapy and are not addressing their needs specifically. The kid in therapy is then being asked `why are you so sad?’ and the kid is like.. `I’m not sad.’ "} -P17, Case Manager, BSW, 8 years}
\end{myquote}
 
This is further problematic because unnecessary services are not only an added financial burden on CWS but they also add to the medical trauma of foster children who are continually being told that something is wrong with them. Finally, as previously noted, services assigned through an isolated view of a child might be less effective than family-level interventions developed through a trauma-informed perspective. Algorithms like CANS, however, limit child-welfare workers from using their expertise and developing more family-centered practices.

%==========================================================================================
%Administrative data curated thorugh bureaucratic processes cannot be uncritically used 


\subsubsection{Algorithmic Decision-Support Systems and Bureaucratic Processes Need to be Aligned.} In this section, we discuss the themes around the benefits and drawbacks that emerged when balancing the ADMAPS dimensions of algorithmic decision-making and bureaucratic processes. 

\vspace{0.2cm}
\textbf{When algorithmic decision-making and bureaucratic processes are aligned, it can help train caseworkers.} Most participants (70\%, n=14) recognized the value of algorithms as essential training mechanisms. Continuous engagement with 7ei in trauma-informed meetings under proper supervision ensures that caseworkers are continually having conversations centered in trauma and are coming up with solutions founded in TIC. This is essential because CWS suffers from a high turnover with lack of adequate training and supervision being some of the leading causes \cite{carnochan2013achieving}. During the observations, experienced members of the child-welfare team such as the supervisors and permanency consultants brainstormed ideas with the caseworkers using 7ei and shared practices and approaches that had worked in the past with other families. A program director explained:

\begin{myquote}
    \textcolor{mygray}{\textit{"It [7ei] makes us think differently and in the moment think through TIC [trauma-informed care].. what is the impact of that [incident]? How can we help support parents and children and help with emotional regulation? What can we do to build their relationships and how do we support the people in their life so that they show better caregiver capacity to manage what this child is going through"} -P7, Child Welfare Program Director, MSW, 20 years}
\end{myquote}

7ei meetings are also attended by Caregiver Support Specialists and Family Preservation Specialists who based on case circumstances also offer their expertise to the caseworkers on how to proceed. Several participants (70\%, n=14) also recognized the Anti Sex-Trafficking algorithm as a good training tool such that caseworkers are always aware of and looking for red flags associated with sex-trafficking. This tool is also used in a team-setting and allows for the less experienced caseworkers to learn from the seasoned members of the team in how to perceive certain risks as well as how to follow up on them without confronting the foster youth. One supervisor explained: 

\begin{myquote}
    \textcolor{mygray}{\textit{"Its a whole change of mindset and and we’re now more cognizant of some of those red flags. So I appreciate that. So, anytime in supervision, if they [caseworkers] start talking about some of these things, we pull up the tool and go through it and start discussing how to proceed"} -P15, Child Welfare Supervisor, 9 years}
\end{myquote}

However, participants who found great value in the Anti Sex-Trafficking algorithm as a training mechanism were also equally frustrated by the mandatory reporting nature of it. 
%------------------------------------------

\vspace{0.1cm}
\textbf{When the algorithmic decision-support system is not aligned with the constraints of the bureaucratic system, it leads to utility issues.} The utility of algorithmic decision-support systems is severely limited when they do not account for the organizational constraints within which they must operate. This challenge and frustrations on part of caseworkers was observed in 80\% (n=16) of the interviews, 73\% (n=11) of the planning meetings, and 82\% (n=32) of the permanency consultations. Most of the participants (80\%, n=16) stated that they were unable to use algorithms as intended because of several organizational constraints such as limited time availability due to high caseloads. For instance, properly conducting CANS requires the caseworkers to interviews several individuals such as the foster parents, relatives, and teachers to be able to get consistent information. However, most caseworkers have high caseloads and do not have enough time to devote towards properly conducting each assessment. A permanency consultant explained: 

\begin{myquote}
    \textcolor{mygray}{\textit{"It can take hours to properly do CANS. Everyone is stretched too thin.. we literally do not have the time to do that."} -P2, Permanency Consultant, MSW, 20 years}
\end{myquote}

Moreover, the bureaucratic policy that requires CANS to be conducted every six months makes it unfeasible for caseworkers to interview anyone beyond the foster parents. However, as previously noted, the assessment is also tied to the compensation offered to foster parents which further leads to foster parents exaggerating child behaviors. A supervisor explained that the algorithm did not need to be manipulated and caseworkers could request an exceptional rate to account for several different factors such as transportation services, therapy, school activities etc. However, she also explained that high caseloads make it hard to devote any extra time to each assessment:

\begin{myquote}
    \textcolor{mygray}{\textit{"The supervisor or worker can take a little extra time and put an exceptional amount in. But again, everybody has too much to get done and it’s unlikely for somebody to even think about that until they are in the middle of submitting CANS and its due the next day."} -P8, Child Welfare Supervisor, MSW, CAPSW, 19 years}
\end{myquote}

Caseworkers who continue to feel disempowered and frustrated by CANS find it easier to manipulate CANS scores to produce a higher rate than request the addition of an exceptional rate which needs to be approved by the supervisor. Most participants (75\%, n=15) also shared significant concerns about the fidelity of data being used to develop algorithms. Administrative data curated through bureaucratic processes can not be uncritically used to develop algorithms. Participants shared that the data about families is collected by caseworkers and it was hard to acquire accurate information. Oftentimes, caseworkers might receive conflicting information from parents, relatives, and neighbors. A supervisor explained:

\begin{myquote}
    \textcolor{mygray}{\textit{"People aren’t willing to happily share personal information about themselves. And understandably so. It’s really hard to be able to get consistent information to be able to put in some data system to bust out a decision. So I find this really difficult to comprehend how we would even consider that"} - -P13, Child Welfare Supervisor, MSW, 12 years}
\end{myquote}

Families view caseworkers as representatives of the state and are unwilling to trust them or share any information that they might consider incriminating. Therefore, much of the information is based on the caseworker's perception of the family. This problem is further exacerbated by the fact that most caseworkers are new graduates and lack adequate experience. A program director explained that during investigations, caseworkers need to ask the right questions, read situations, and follow-up to be able to derive meaningful information. However, caseworkers acquire these skills through years of experience.

%------------------------------------------

\vspace{0.1cm}
\textbf{If the algorithms are not explained well to the practitioners, they don’t trust them.} Most of the participants (85\%, n=17) were unaware of the algorithms being used. They did not recognize CANS or 7ei as algorithmic systems, even though they interact with them on a daily basis. This finding is especially interesting because the CANS training material recognizes it as an algorithm and explicitly lays out the purposes (i.e. - outcomes) that the algorithm is designed to accomplish. CWS started using algorithms as a means to track important performance metrics such as permanency and placement stability as mandated by federal legislation \cite{wilson2014integrating}. Moreover, several psychometric assessments that are routinely used in child-welfare to assess the risks and needs of children and parents have adopted algorithmic analogues in the form of risk assessment algorithms. They are now being used as data collectors for all cases as well as decision arbiters for future cases. The CANS algorithm is a case in point of this scenario which is an algorithmic version of the CANS communimetric assessment \cite{lyons2009communimetrics} and has been re-purposed for other outcomes. Interestingly, caseworkers were well aware of assessments used at the agency but did not actively recognize the algorithmic components unless the interviewer nudged them to think about some of the automated aspects. For instance, when explicitly discussing CANS, all the interviewees realized it to be an algorithm that plays a pertinent role in decision-making. We asked a permanency consultant how she thought CANS worked and she exclaimed: 

\begin{myquote}
    \textcolor{mygray}{\textit{"Yes, okay! Right! Because we put in the scores, and it generates the rate. Oh and I hate the CANS! I, I’ve expressed it a lot of times that CANS should not be tied to money."} -P6, Permanency Consultant, BSW, 3 years}
\end{myquote}

As soon as participants recognized the automated decision-making aspects of these decision tools, they started to share some other ambiguous aspects. For instance, they had trouble recognizing who managed these decision-tools and shared that different tasks associated with these tools were distributed across the agency. Most of the participants (85\%, n=17) where unable to isolate CANS to a particular role or "place". CANS is embedded in several aspects of the case planning process with different departments involved. Case management team focuses on assessing risks and needs whereas the data specialists track scores, and the fiscal liaisons review and approve foster parent compensations. Participants (70\%, n=14) also alluded to the fact that algorithms meant different things to people based on their intended goals. For instance, one permanency consultant asserted:

\begin{myquote}
    \textcolor{mygray}{\textit{"Case management try to do a good job with risks and needs but of-course foster parents only care about the rate. I know X’s team [data specialists] look at scores to see if there is improvement. But there is also Y [fiscal liaison] who just wants the scores to be turned in on time so that he doesn’t have to chase people down"} -P1, Permanency Consultation Supervisor, MSW, APSW, 22 years}
\end{myquote}
 
Several participants (75\%, n=15) recognized that CANS, AST, and LPS decision tools meant different things in different contexts. Lack of awareness about algorithms at the organizational level and their distributed nature augmented caseworkers’ distrust.
%For instance, the clinical therapist viewed CANS as a communication tool used to shared information about children. In contrast, some caseworkers viewed CANS as a service-planning tool while others used it strictly as a rate-setting tool.

%=============================================

\subsubsection{Collective Buy-in Requires Trust in Outcomes at Both the Caseworker and Bureaucratic Levels.} In this section, we discuss the themes around the benefits and drawbacks that emerged when balancing the ADMAPS dimension of human discretion and bureaucratic processes with respect to decision outcomes that the CWS agency implements.

\vspace{0.2cm}
\textbf{When the algorithmic outcomes miss important context, practitioners don’t trust them} This challenge emerged in 70\% (n=14) of the interviews, 67\% (n=10) of the planning meetings and 75\% (n=30) of the permanency consultations. Algorithms attempt to generalize child and family characteristics and place them in certain categories to be able to make a determination. However, this inadvertently leads to a loss of information with respect to the final outcome since all the information cannot be accounted for by these algorithms. For instance, the CANS algorithmic assessment focuses on child behaviors, risks, and needs based on the last 30 days and does not account for traumatic triggers that can lead to serious emotional dysregulation from time to time. A permanency consultant explained:

\begin{myquote}
    \textcolor{mygray}{\textit{"CANS does not account for trauma in the way 7ei does. We have a child that goes into manic depression every year around holiday season and needs to be cared for 24/7. So, one of the foster parents has to quit their job. However, there is no way to account for that in CANS. This child is doing fine right now but we know that traumatic trigger is coming."} -P3, Permanency Consultant, MSW, APSW, 9 years}
\end{myquote}

Participants shared similar concerns about the Anti Sex-Trafficking tool. Participants (65\%, n=13) shared that the tool was useful to identify risk factors, however, the presence of risk factors does not necessarily mean that the foster youth is being trafficked. A supervisor explained:

\begin{myquote}
    \textcolor{mygray}{\textit{"We have a 12 year old boy who suffers from a lot of sexual trauma. He met a bunch of criteria on the tool and we had to report to HART. We have been with this boy for many years.. we know him and what his behaviors are connected to. Reporting to HART felt very odd"} -P11, Child Welfare Supervisor, MSW, APSW, 9 years}
\end{myquote}

Here, the supervisor alludes to the fact that presence of risk factors did not capture the full picture and missed important context about what is going on with this child. As previously discussed, child-welfare teams are having on-going conversations about the risk of sex-trafficking from the onset of a case and are able to investigate concerns without reporting to HART. Continued interactions illustrated by these examples leads to an accumulation of distrust towards algorithms that often miss important nuances and context.

%Participants (55\%, n=11) also recognized that the 7ei algorithm added a contextual lens that placed trauma front and center and allowed for the team to deliberate over the underlying trauma and brainstorm ideas on how to address it. However, there are several instances where 7ei also misses out on important context because of the categorical rating of 7ei domains. For instance, at a meeting, a case manager asked if she could rate Perspective Shift as a 2.5 since she did not think the parents could be rated either a 2 (lacks understand of trauma) or a 3 (understands trauma exposure). In such cases, the teams go with the lower rating, however, that also negates any progress that the case manager might have made while working with the family. Continued interactions illustrated by these examples leads to an accumulation of distrust towards these algorithms that often miss important nuances and context.

%---------------------

\vspace{0.1cm}
\textbf{There is collective buy-in when practitioners believe that better outcomes are being achieved.}
This theme emerged in 85\% (n=17) of the interviews, 67\% (n=10) of the planning meetings, and 62.5\% (n=25) of the permanency consultations. Participants appreciated 7ei and trauma-informed care because it allowed them to directly help families by developing specific plans for them. Moreover, they were aware that trauma-responsive services developed through TIC lead to better permanency and placement outcomes for children. When frustrated by algorithms such as CANS, caseworkers often asked why they were still expected to use CANS when 7ei was leading to better outcomes. 

The agency developed a comprehensive four-part evidence-based service program centered in trauma-informed care of which the algorithmic tool is just one component. The first component of this program involves extensive ongoing TIC trainings. The second component introduced child-welfare staff to trauma-informed assessments that resulted in family-level interventions. The third component was the availability of specialized supervision and consultations provided by a clinical supervisor, TIC program administrator, medical expert, and a caregiver support specialist. Finally, the fourth component of this program is the 7ei algorithm which allows the child-welfare team to break down each case into seven domains and apply TIC principles and practices to it. In sum, the agency significantly invested in resources to ensure that TIC practice and 7ei were fully-supported by bureaucratic processes. A better understanding of what a family might be going through at a psychological level and knowing exactly how to help them has led to the collective buy-in from caseworkers. Most participants (85\%, n=17) found great value in TIC and appreciated 7ei as a tool designed to be a guiding framework for TIC. One permanency consultant explained:

\begin{myquote}
    \textcolor{mygray}{\textit{"Compassion fatigue in child welfare is very real. This tool has helped me truly understand what trauma can do to the brain. So I think now that we have a better understanding of trauma... we also have more empathy, and we go the extra mile to help families."} -P1, Permanency Consultation Supervisor, MSW, APSW, 22 years}
\end{myquote}
 
This was also evident at the meetings where the child-welfare staff urged case managers to ask and think in terms of \textit{"What happened to you and how can I help you?"} instead of \textit{"What is wrong with you?"} when working with children and families. That is, having a perspective shift and thinking in terms of the impact of trauma and not just exhibited behaviors. Moreover, a study published by independent researchers showed that child-welfare teams who implemented TIC practices using 7ei exhibited improved permanency and placement stability outcomes for their cases. This has further deepened the collective buy-in from caseworkers who often brought up the "study" to state that their practice centered in TIC worked and lead to better outcomes, and therefore, the legal parties needed to trust their judgments more. However, interestingly, none of the participants except the program director were able to locate the study and share it with us.

%---------------------

\vspace{0.1cm}
\textbf{Lack of trust in algorithmic outcomes, leads to concerns about unethical and unsound decision-making.}
This theme emerged in 80\% (n=16) of the interviews, 40\% (n=6) of the planning meetings, and 45\% (n=18) of the permanency consultations where participants recognized that algorithms in use sometimes led them to make unethical or unsound decisions. Surprisingly, even though 90\% (n=18) of the participants recognized that caseworkers were gaming the system to produce higher compensations, some participants (40\%, n=8) did not consider the decisions made to be unethical or unsound. To them, this is how the system was set up to be used. With contradictory incentive structures and conflicting values, caseworkers are often put in a position where they are forced to make such decisions. As previously discussed, both caseworkers and foster parents are co-opting CANS to produce a higher compensation, however, most participants (90\%, n=18) recognized that the base compensation offered to foster parents is pretty low and gaming the algorithm was the only convenient way to produce an adequate rate. A supervisor explained:

\begin{myquote}
    \textcolor{mygray}{\textit{ "There is a lack of good foster homes and there is no financial incentive to be doing this work... So caseworkers do whatever they can to get them [foster parents] the money they need or we risk disrupting a placement...Several foster parents have put in notices in the past because they can’t financially sustain the placement"} -P9, Child Welfare Supervisor, MSW, 13 years}
\end{myquote}

% Nonetheless, some supervisors have devised their own fairness strategies against excessive gaming to ensure that all foster parents are being paid consistently with respect to the needs of foster children. One supervisor stated:

% \begin{myquote}
%     \textcolor{mygray}{\textit{"CANS assessments are always rushed. But when I do CANS, I look at the old one. I copy it over and then I follow up to see if anything changed? And then I try to stay consistent across. If I give \$100 for this particular child, what is different from another child that has those same needs? Because it’s not fair for one kid to get a higher rate than another one, but it is definitely subjective."} -P8, Child Welfare Supervisor, MSW, CAPSW, 19 years}
% \end{myquote}

Another challenging aspect of using CANS where it leads to unsound decision-making is that it is now being used to track progress with respect to mental health; an unintended outcome of the continuous data collection. Consequently, an improvement (or deterioration) in mental health is impacting placement decisions. A clinical therapist explained: 

\begin{myquote}
    \textcolor{mygray}{\textit{"Sometimes a kid isn’t doing well because they are working through things. For example, when a kid starts therapy sometimes their behaviors gets worse, but it might actually be that they’re working through some things in therapy. And that’s not captured by the tool. When there is no context, I just can’t interpret whether or not that worsening is actually a bad thing."} -P16, Clinical Therapist, LCSW, 5 years}
\end{myquote}

%Most participants (60\%, n=13) also shared similar concerns in that CANS does not account for traumatic triggers. CANS scores are calculated based on child behaviors over the last 30 days, however, lack of exhibited behaviors does not mean the child has recuperated from trauma exposure. 
These frustrations were also consistent with the fact that CANS is tied to service-planning where CANS recommends unnecessary child-level services when family-level interventions are often more effective in helping the family heal and cope with trauma. Prior studies have found that caseworkers distrust risk assessment algorithms such as CANS because of their deficit-based nature \cite{brown2019toward}. Interestingly, participants who were averse to this deficit-based nature did find value in risk assessment in regard to understanding a family's history. One permanency consultant explained:

\begin{myquote}
    \textcolor{mygray}{\textit{"The data gives you a bigger picture of what the family is going through. Because the families are not always honest with us about what they need. And so if you can see that they were in drug and alcohol services or housing authority... that would be helpful in child welfare. Not necessarily giving them a score. I don’t even know what to do with the score. It tells me nothing."} -P6, Permanency Consultant, BSW, 3 years}
\end{myquote}

Understanding a family’s past helps caseworkers assess the type of services that would be most beneficial for them. Looking at this data from a trauma-informed perspective allows caseworkers to better understand the underlying trauma in the family that might be leading to exhibited behaviors and subsequent interactions with the child-welfare system. This points to a change in mindset in regard to the intended goal of risk assessment of (i.e. - predicting the risk of future harm) towards a strength-based outcome of providing the right services to families and not necessarily labeling them as high or low risk. The permanency consultant here also invokes social work's core value of service and helping families and sees the utility in risk assessment through that perspective.

==> CWS Daily Algorithmic Practices 5.0 Camera Ready (ARXIV)/test.tex <==
Scholars within the Public Administration and Policy field have extensively studied how human discretion by street-level bureaucrats \footnote{A street-level bureaucrat is a professional service worker (e.g., social worker, police officer, teacher) who operates in the frontline of public service provision. They interact closely with clients and makes decisions about them based on how they interpret policies relating to the situations at hand \cite{lipsky2010street}.} plays a central role in navigating bureaucratic processes and implementing policies. For example, bureaucrats act with a certain level of autonomy in how they interpret and apply professional standards when determining which clients must receive welfare benefits or services \cite{sosin2010discretion}. They also use their discretionary power to subvert, supplement, and fill in gaps within legislation \cite{sosin2010discretion, lipsky2010street}. As Lipsky explained, bureaucrats exercise discretion so frequently that they often create policy in practice \cite{lipsky2010street}. Public administration scholars have also started to recognize the impact of information communication technologies (ICTs) on the nature of human discretion and bureaucracy with some recent attention paid to artificial intelligence \cite{busch2018digital, peeters2020agency, m2020artificial, bullock2019artificial}. However, several of these studies, rich in their understanding of human discretion and bureaucracy, continue to treat algorithms as peripheral end products; a new part of bureaucracy to which human discretion must adapt. The CSCW and broader HCI community has a long history of unpacking algorithmic systems as well as building more human-centered \cite{baumer2017toward} and value-sensitive versions \cite{zhu2018value}.

Science and Technologies Studies (STS) scholars conducting studies in the public sector have used Kitchin and Lauriault's framework of \textit{data assemblages} \cite{kitchin2014towards} to study the politics of data systems \cite{redden2020datafied, williamson2016digital, leszczynski2016speculative}. Data assemblages perceive data systems as complex assemblages of human actors, artifacts, technical systems, institutions and ideas. This provides a means to consider how these systems are socially, economically, and politically constructed. Similarly, STS scholars have also used Seaver’s notion of \textit{algorithms as culture} \cite{seaver2017algorithms} to understand the social implications and values of algorithmic systems through an ethnographic analysis. These studies have made significant contributions towards the community’s understanding of how algorithms shape and are shaped by cultural context, how value is inscribed to algorithms, and how power is afforded to them.  However, within the public sector, there is a need to further explore the complex interdependencies between the core elements of human discretion, bureaucratic processes, and algorithmic decision-making and the dimensions within these elements. HCI scholars have also recognized the pertinent role of bureaucracy with respect to the design of civic technologies \cite{holten2020shifting, dow2018between, lodato2018institutional, light2019breakdown}. There is an appreciation and understanding of bureaucracy with respect to configuring design spaces for participatory design \cite{saxena2020conducting, lodato2018institutional, robertson2020if} but we need to further explore how bureaucracy informs human discretion which then directly impacts how humans interact with algorithmic systems.

Below, we operationalize the distinct dimensions that exist within each of these elements (i.e. - human discretion, bureaucratic processes, and algorithmic decision-making) into a cohesive framework. 


==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> RQ2table.tex <==
%============================== RQ2 =======================================
\begin{table}[]
\Small
\begin{center}
\begin{tabular}{|>{\raggedright}p{3cm}|>{\raggedright}p{5cm}|>{\raggedright\arraybackslash}p{5cm}|}
\hline
\rule{0pt}{1.3em}\cellcolor{mygray3}{\textbf{Framework Dimension}} & \rule{0pt}{1.2em}\cellcolor{mygray3}{\textbf{Positive Exemplar}} & \rule{0pt}{1.2em}\cellcolor{mygray3}{\textbf{Negative Exemplar}}\\
\hline
\multicolumn{3}{|l|}{\rule{0pt}{1.1em}{\textbf{Human Discretion}}}  \\
\hline
Professional Expertise  & \textit{} & \textit{"CANS has become all about the rate with little attention paid to actually helping the child"}\\
\arrayrulecolor{mygray2}\hline
Value Judgments   & \textit{} & \textit{"Caseworkers feel pressured to rate CANS higher to produce a higher compensation for foster parents"}\\
\arrayrulecolor{mygray2}\hline
Heuristic Decision-Making    & \textit{"Every case is different.. with 7ei we can focus on what's important for each case whether it's focusing on a child's trauma or parents' caregiver capacity"} &\\
\arrayrulecolor{black}\hline
\multicolumn{3}{|l|}{\rule{0pt}{1.1em}{\textbf{Algorithmic Decision-Making}}} \\
\hline
Relevant Data    & \textit{} & \textit{"CANS is frustrating because it lacks context about what’s going on with the child. It doesn’t account for the social structures that the kid interacts in."}\\
\arrayrulecolor{mygray2}\hline
Type of Decision-Support    & \textit{} & \textit{"Rate is generated by itself after we put in the CANS scores"}\\
\arrayrulecolor{mygray2}\hline
Degree of Uncertainty & \textit{""} & \textit{""}\\
\arrayrulecolor{black}\hline
\multicolumn{3}{|l|}{\rule{0pt}{1.1em}{\textbf{Bureaucratic Processes}}} \\
\hline
Resources \& Constraints  & & \\
\arrayrulecolor{mygray2}\hline
Admin. \& Training  & \textit{} &\\
\arrayrulecolor{mygray2}\hline
Laws \& Policies    & \textit{} &\\
\arrayrulecolor{black}\hline

\end{tabular}
\end{center}
\caption{RQ2: Balancing dimensions of framework}
\vspace{-0.3cm}
\end{table}
%============================== RQ2 =======================================

==> RQ3table.tex <==
%============================== RQ3 =======================================
\begin{table}[]
\Small
\begin{tabular}{|>{\raggedright}p{5cm}|>{\raggedright}p{6cm}|>{\raggedright\arraybackslash}p{2cm}|}
\hline
\rule{0pt}{1.3em}\cellcolor{mygray3}{\textbf{Theme}} & \rule{0pt}{1.2em}\cellcolor{mygray3}{\textbf{Illustrative Quotation}} & \rule{0pt}{1.2em}\cellcolor{mygray3}{\textbf{Codes}} \\
\hline
\multicolumn{3}{|c|}{\rule{0pt}{1.1em}{\textbf{Algorithmic decision-making should seek to augment human discretion rather than attempt to replace it 
}}}  \\
\hline
When aligned, algorithms augments decision-making processes, but a lack of alignment can takeaway autonomy and heuristic decision-making (85\%, n=17) & \textit{"7ei is embedded in the agency. Everything is based in the trauma-responsive model and often caseworkers are working through 7ei domains without even realizing it"} & values, heuristics, autonomy, discretion\\
\arrayrulecolor{mygray2}\hline
When aligned, algorithms can help embed important value judgments into the decision-making process (65\%, n=13) & \textit{"It [7ei] allows us to look at the case from the child's perspective and not just our own perspective. We might not trust mom but the child adores her. So we need to work with her and build that relationship"} & negotiate values, balance needs, personalized care\\
\arrayrulecolor{mygray2}\hline
Algorithms replacing the need for caseworker expertise can lead to inadequate and unreliable decision-making (70\%, n=14)
    & \textit{"We are reporting cases to HART just based on some risk factors on a checklist [AST]. It's not the full picture and only frustrates HART"} & lack of heuristics, high pressure, futile services\\
\arrayrulecolor{black}\hline
\multicolumn{3}{|l|}{\rule{0pt}{1.1em}{\textbf{Algorithmic decision-support systems and bureaucratic processes need to be aligned
}}} \\
\hline
When algorithmic decision-making and bureaucratic processes are aligned, it can help train caseworkers  (70\%, n=14)
  & \textit{"Every case is centered in the trauma-responsive model using 7ei. It ensures that caseworkers are always thinking through TIC"} & team expertise, supervision, engagement\\
\arrayrulecolor{mygray2}\hline
When the algorithmic decision-support system is not aligned with the constraints of the bureaucratic system, it leads to utility issues  (80\%, n=16)
   & \textit{"There are restrictions on how it [LPS] is used. You can’t rate a placement to be 'Good’ because you don’t have a court date set. But the hearing can go either way. We don't control that"} & time pressure, data fidelity, gaming the tool\\
\arrayrulecolor{mygray2}\hline
If the algorithms are not explained well to the professionals, they don’t trust them (70\%, n=14)
 & \textit{"[LPS] It's all perspective. Different people can be looking at the same issues, and have different reasons for saying the placement is 'good' or 'poor'"} & implicit use, hard to locate, other meanings\\
\arrayrulecolor{black}\hline
\multicolumn{3}{|l|}{\rule{0pt}{1.1em}{\textbf{Collective buy-in requires trust in algorithmic outcomes at both the caseworker and bureaucratic levels
}}} \\
\hline
When the algorithms miss important context, people don’t trust them (70\%, n=14)
  & \textit{"CANS does not account for underlying trauma or a child's support system.. which is essential"} & trauma, reductive, relationships\\
\arrayrulecolor{mygray2}\hline
There is collective buy-in when people feel like it leads to better outcomes (85\%, n=17)
 & \textit{"7ei scores show that trauma-informed meetings are actually leading to better placement stability and permanency outcomes"} & TIC practice, better outcomes, value-centered\\
\arrayrulecolor{mygray2}\hline
Lack of trust in algorithmic outcomes, leads to concerns about unethical and unsound decision-making (80\%, n=16)
   & \textit{"If several behaviors are scored high on CANS then that is a clear indicator that the caseworker was only trying to generate a higher rate"} & manipulate outcomes, lack of progress\\
\arrayrulecolor{black}\hline

\end{tabular}
\caption{RQ3: Benefits and Drawbacks of balancing Human Discretion, Algorithmic Decision-Making, and Bureaucratic Processes}
\label{RQ3:codebook}
\vspace{-0.8cm}
\end{table}
%============================== RQ3 =======================================

==> test.tex <==
Scholars within the Public Administration and Policy field have extensively studied how human discretion by street-level bureaucrats \footnote{A street-level bureaucrat is a professional service worker (e.g., social worker, police officer, teacher) who operates in the frontline of public service provision. They interact closely with clients and makes decisions about them based on how they interpret policies relating to the situations at hand \cite{lipsky2010street}.} plays a central role in navigating bureaucratic processes and implementing policies. For example, bureaucrats act with a certain level of autonomy in how they interpret and apply professional standards when determining which clients must receive welfare benefits or services \cite{sosin2010discretion}. They also use their discretionary power to subvert, supplement, and fill in gaps within legislation \cite{sosin2010discretion, lipsky2010street}. As Lipsky explained, bureaucrats exercise discretion so frequently that they often create policy in practice \cite{lipsky2010street}. Public administration scholars have also started to recognize the impact of information communication technologies (ICTs) on the nature of human discretion and bureaucracy with some recent attention paid to artificial intelligence \cite{busch2018digital, peeters2020agency, m2020artificial, bullock2019artificial}. However, several of these studies, rich in their understanding of human discretion and bureaucracy, continue to treat algorithms as peripheral end products; a new part of bureaucracy to which human discretion must adapt. The CSCW and broader HCI community has a long history of unpacking algorithmic systems as well as building more human-centered \cite{baumer2017toward} and value-sensitive versions \cite{zhu2018value}.

Science and Technologies Studies (STS) scholars conducting studies in the public sector have used Kitchin and Lauriault's framework of \textit{data assemblages} \cite{kitchin2014towards} to study the politics of data systems \cite{redden2020datafied, williamson2016digital, leszczynski2016speculative}. Data assemblages perceive data systems as complex assemblages of human actors, artifacts, technical systems, institutions and ideas. This provides a means to consider how these systems are socially, economically, and politically constructed. Similarly, STS scholars have also used Seaver’s notion of \textit{algorithms as culture} \cite{seaver2017algorithms} to understand the social implications and values of algorithmic systems through an ethnographic analysis. These studies have made significant contributions towards the community’s understanding of how algorithms shape and are shaped by cultural context, how value is inscribed to algorithms, and how power is afforded to them.  However, within the public sector, there is a need to further explore the complex interdependencies between the core elements of human discretion, bureaucratic processes, and algorithmic decision-making and the dimensions within these elements. HCI scholars have also recognized the pertinent role of bureaucracy with respect to the design of civic technologies \cite{holten2020shifting, dow2018between, lodato2018institutional, light2019breakdown}. There is an appreciation and understanding of bureaucracy with respect to configuring design spaces for participatory design \cite{saxena2020conducting, lodato2018institutional, robertson2020if} but we need to further explore how bureaucracy informs human discretion which then directly impacts how humans interact with algorithmic systems.

Below, we operationalize the distinct dimensions that exist within each of these elements (i.e. - human discretion, bureaucratic processes, and algorithmic decision-making) into a cohesive framework. 

